Purely flavor-changing Z' bosons and where they might hide

A plethora of ultraviolet completions of the Standard Model have extra U(1) gauge symmetries. In general, the associated massive $Z^\prime$ gauge boson can mediate flavor-changing neutral current processes at tree level. We consider a situation where the $Z^\prime$ boson couples solely via flavor-changing interactions to quarks and leptons. In this scenario the model parameter space is, in general, quite well constrained by existing flavor bounds. However, we argue that cancellation effects shelter islands in parameter space from strong flavor constraints and that these can be probed by multipurpose collider experiments like ATLAS or CMS as well as LHCb in upcoming runs at the LHC. In still allowed regions of parameter space these scenarios may help to explain the current tension between theory and experiment of $(g-2)_\mu$ as well as a small anomaly in $\tau$ decays.

==> out <==
This is pdfTeX, Version 3.14159265-2.6-1.40.15 (TeX Live 2015/dev/Debian) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./submit2.tex
LaTeX2e <2014/05/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size11.clo))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/appendix/appendix.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/cite/cite.sty)
(/usr/share/texmf/tex/latex/feynmf/feynmp.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg)))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texlive/texmf-dist/tex/latex/cleveref/cleveref.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/epsfig.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty))
(/usr/share/texlive/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/changepage/chngpage.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/lipsum/lipsum.sty) (./submit2.aux)
(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./submit2.out) (./submit2.out)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd) [1{/var/lib/texmf/fo
nts/map/pdftex/updmap/pdftex.map}] [2]
Underfull \hbox (badness 10000) in paragraph at lines 255--262

[3] <figures/bsem_750.pdf, id=204, 578.16pt x 433.62pt>
<use figures/bsem_750.pdf> [4]
<figures/bsmt_750.pdf, id=222, 578.16pt x 433.62pt> <use figures/bsmt_750.pdf>
<figures/bdem_750.pdf, id=225, 578.16pt x 433.62pt> <use figures/bdem_750.pdf>
[5 <./figures/bsem_750.pdf>] [6 <./figures/bsmt_750.pdf>] [7 <./figures/bdem_75
0.pdf>] <figures/sig_lim8_em.pdf, id=524, 578.16pt x 433.62pt>
<use figures/sig_lim8_em.pdf>
<figures/projection.pdf, id=525, 578.16pt x 433.62pt>
<use figures/projection.pdf>
Overfull \hbox (2.43332pt too wide) in paragraph at lines 501--518
[]$[]$ $[]$ 
[8 <./figures/sig_lim8_em.pdf> <./figures/projection.pdf

pdfTeX warning: pdflatex (file ./figures/projection.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
>] [MP to PDF] (./mesonmix_zp.1) (./mesonmix_zp.t1) [MP to PDF]
(./mesonmix_zp.2) (./mesonmix_zp.t2)
<figures/bsem_mix_750.pdf, id=664, 578.16pt x 433.62pt>
<use figures/bsem_mix_750.pdf> [9] [10 <./figures/bsem_mix_750.pdf>] [11]
[12] [MP to PDF] (./kp2pip_sm.1) (./kp2pip_sm.t1) [MP to PDF] (./kp2pip_sm.2)
(./kp2pip_sm.t2) [MP to PDF] (./kp2pip_sm.3) (./kp2pip_sm.t3) [MP to PDF]
(./kp2pip_zp.1) (./kp2pip_zp.t1) [13] [MP to PDF] (./kp2pi0.1) (./kp2pi0.t1)
[14]
Underfull \hbox (badness 10000) in paragraph at lines 1138--1149

[MP to PDF] (./b0nunu.1) (./b0nunu.t1) [MP to PDF] (./b0nunu.2) (./b0nunu.t2)
[15] [MP to PDF] (./bp2kp.1) (./bp2kp.t1) [16] [MP to PDF] (./lep_dec.1)
(./lep_dec.t1) [MP to PDF] (./lep_dec.2) (./lep_dec.t2)

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1414.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\mu' on input line 1414.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1414.

[17]

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1434.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\tau' on input line 1434.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1434.

[18] [MP to PDF] (./tree_mix.1) (./tree_mix.t1) [MP to PDF] (./tree_mix.2)
(./tree_mix.t2) [19] [20] [MP to PDF] (./tree_lep.1) (./tree_lep.t1)
<figures/xsec750_et.pdf, id=985, 578.16pt x 433.62pt>
<use figures/xsec750_et.pdf>
Overfull \hbox (2.43332pt too wide) in paragraph at lines 1676--1710
[]$[]$ $[]$ 
[21] [22 <./figures/xsec750_et.pdf>]

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1765.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `superscript' on input line 1765.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\prime' on input line 1765.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1765.

[23]

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1841.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `superscript' on input line 1841.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\prime' on input line 1841.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1841.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1841.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1841.

[MP to PDF] (./zp_triangle.1) (./zp_triangle.t1) [24]
Underfull \hbox (badness 10000) in paragraph at lines 1915--1924


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1942.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 1942.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\mu' on input line 1942.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1942.

<figures/rh_bsmt_200.pdf, id=1119, 578.16pt x 433.62pt>
<use figures/rh_bsmt_200.pdf>
<figures/rh_g_2.pdf, id=1120, 578.16pt x 433.62pt> <use figures/rh_g_2.pdf>
Overfull \hbox (2.43332pt too wide) in paragraph at lines 1947--1962
[]$[]$ $[]$ 
<figures/bsmt_ax_1500.pdf, id=1121, 578.16pt x 433.62pt>
<use figures/bsmt_ax_1500.pdf>
<figures/ax_g_2.pdf, id=1122, 578.16pt x 433.62pt> <use figures/ax_g_2.pdf>
Overfull \hbox (2.43332pt too wide) in paragraph at lines 1968--1984
[]$[]$ $[]$ 

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1998.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 1998.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\mu' on input line 1998.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1998.

[25] [26 <./figures/rh_bsmt_200.pdf> <./figures/rh_g_2.pdf

pdfTeX warning: pdflatex (file ./figures/rh_g_2.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
> <./figures/bsmt_ax_1500.pdf

pdfTeX warning: pdflatex (file ./figures/bsmt_ax_1500.pdf): PDF inclusion: mult
iple pdfs with page group included in a single page
> <./figures/ax_g_2.pdf

pdfTeX warning: pdflatex (file ./figures/ax_g_2.pdf): PDF inclusion: multiple p
dfs with page group included in a single page
>]

Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 2032.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 2032.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `\mu' on input line 2032.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 2032.

[27] [MP to PDF] (./loop_mix.1) (./loop_mix.t1) [MP to PDF] (./loop_mix.2)
(./loop_mix.t2) [28]
Underfull \hbox (badness 10000) in paragraph at lines 2178--2193


Underfull \hbox (badness 10000) in paragraph at lines 2196--2210


Underfull \hbox (badness 10000) in paragraph at lines 2213--2229

[29] [30] <figures/1tev/bsem1.pdf, id=1463, 578.16pt x 433.62pt>
<use figures/1tev/bsem1.pdf>
<figures/1tev/bdem1.pdf, id=1464, 578.16pt x 433.62pt>
<use figures/1tev/bdem1.pdf>
<figures/1tev/sdem1.pdf, id=1465, 578.16pt x 433.62pt>
<use figures/1tev/sdem1.pdf>
<figures/1tev/cuem1.pdf, id=1466, 578.16pt x 433.62pt>
<use figures/1tev/cuem1.pdf>
Overfull \hbox (83.80849pt too wide) in paragraph at lines 2380--2400
[]$[]$ $[]$ 

Overfull \hbox (83.80849pt too wide) in paragraph at lines 2380--2400
[]$ $[]$ 
<figures/1tev/bset1.pdf, id=1469, 578.16pt x 433.62pt>
<use figures/1tev/bset1.pdf>
<figures/1tev/bdet1.pdf, id=1470, 578.16pt x 433.62pt>
<use figures/1tev/bdet1.pdf>
<figures/1tev/sdet1.pdf, id=1471, 578.16pt x 433.62pt>
<use figures/1tev/sdet1.pdf>
<figures/1tev/cuet1.pdf, id=1472, 578.16pt x 433.62pt>
<use figures/1tev/cuet1.pdf>
Overfull \hbox (83.80849pt too wide) in paragraph at lines 2418--2438
[]$[]$ $[]$ 

Overfull \hbox (83.80849pt too wide) in paragraph at lines 2418--2438
[]$ $[]$ 
<figures/1tev/bsmt1.pdf, id=1475, 578.16pt x 433.62pt>
<use figures/1tev/bsmt1.pdf>
<figures/1tev/bdmt1.pdf, id=1476, 578.16pt x 433.62pt>
<use figures/1tev/bdmt1.pdf>
<figures/1tev/sdmt1.pdf, id=1477, 578.16pt x 433.62pt>
<use figures/1tev/sdmt1.pdf>
<figures/1tev/cumt1.pdf, id=1478, 578.16pt x 433.62pt>
<use figures/1tev/cumt1.pdf>
Overfull \hbox (83.80849pt too wide) in paragraph at lines 2455--2475
[]$[]$ $[]$ 

Overfull \hbox (83.80849pt too wide) in paragraph at lines 2455--2475
[]$ $[]$ 
[31]

LaTeX Warning: Text page 32 contains only floats.


Overfull \vbox (0.17477pt too high) has occurred while \output is active
[32 <./figures/1tev/bsem1.pdf> <./figures/1tev/bdem1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/bdem1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/sdem1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/sdem1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/cuem1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/cuem1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
>] [33 <./figures/1tev/bset1.pdf> <./figures/1tev/bdet1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/bdet1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/sdet1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/sdet1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/cuet1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/cuet1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
>] [34 <./figures/1tev/bsmt1.pdf> <./figures/1tev/bdmt1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/bdmt1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/sdmt1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/sdmt1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
> <./figures/1tev/cumt1.pdf

pdfTeX warning: pdflatex (file ./figures/1tev/cumt1.pdf): PDF inclusion: multip
le pdfs with page group included in a single page
>] [35] [36] [37] [38] (./submit2.aux) )
(see the transcript file for additional information)</usr/share/texlive/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texlive/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmbx12.pfb></usr/share/texlive/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmcsc10.pfb></usr/share/texlive/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmex10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/
amsfonts/cm/cmmi10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmmi12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/
cmmi6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi7.p
fb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></us
r/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi9.pfb></usr/share
/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/share/texliv
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/share/texlive/texmf
-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb></usr/share/texlive/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmr8.pfb></usr/share/texlive/texmf-dist/fonts/type
1/public/amsfonts/cm/cmr9.pfb></usr/share/texlive/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/
cmsy7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy8.p
fb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy9.pfb></us
r/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></usr/shar
e/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmtt10.pfb></usr/share/texl
ive/texmf-dist/fonts/type1/public/amsfonts/symbols/msam10.pfb>
Output written on submit2.pdf (38 pages, 1643000 bytes).
Transcript written on submit2.log.

